An Interdisciplinary Outlook on Large Language Models for Scientific Research

In this paper, we describe the capabilities and constraints of Large Language Models (LLMs) within disparate academic disciplines, aiming to delineate their strengths and limitations with precision. We examine how LLMs augment scientific inquiry, offering concrete examples such as accelerating literature review by summarizing vast numbers of publications, enhancing code development through automated syntax correction, and refining the scientific writing process. Simultaneously, we articulate the challenges LLMs face, including their reliance on extensive and sometimes biased datasets, and the potential ethical dilemmas stemming from their use. Our critical discussion extends to the varying impacts of LLMs across fields, from the natural sciences, where they help model complex biological sequences, to the social sciences, where they can parse large-scale qualitative data. We conclude by offering a nuanced perspective on how LLMs can be both a boon and a boundary to scientific progress.

==> readiness.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{table}[h]
\centering
\scalebox{0.9}{
\begin{threeparttable}
\caption{Readiness Evaluation of \acp{LLM} in Scientific Research}
\label{table:readiness}
\small
\begin{tabular}{ll|cccc}
\hline\hline
                 &                           & Physical Sciences$^{a}$ & Social Sciences$^{b}$ & Engineering$^{c}$ & \multirow{2}{3em}{Example Models}                                    \\
\multicolumn{2}{c|}{Tasks}                                     & \begin{tabular}[c]{@{}l@{}}Astronomy\\Biology\\Physics\end{tabular}           & \begin{tabular}[c]{@{}l@{}}Economics\\...\end{tabular}         & \begin{tabular}[c]{@{}l@{}}Aerospace\\Mechanical\\...\end{tabular}   &                                                                   \\
\hline
%\multirow{2}{5em}{Ideation}    
%                 & Ideation          & 1                    &  1               &               &                 \begin{tabular}[c]{@{}c@{}}a: ProtGPT2 \cite{ProtGPT2}, \\AutoGPT\end{tabular}                                                  \\
%                 & \begin{tabular}[c]{@{}l@{}}Model \&\\Parameter Selection\end{tabular}         & 1                  & 1                  &    1            &                                                \\

\hline
\multirow{2}{5em}{Ideation and Information Review} 
                 & Ideation          & 1                    &  1               &               &                 \begin{tabular}[c]{@{}c@{}}a: ProtGPT2 \cite{ProtGPT2}, \\AutoGPT\end{tabular}                                                  \\
                 & Information Retrival      & 2                    & 2                  & 2              & \begin{tabular}[c]{@{}c@{}}a: astroBERT \cite{astroBERT},  \\ TaxoNERD \cite{TaxoNERD} \end{tabular}  \\
%                 & Literature Review       & 1                    & 1                  & 1              &                                                                   \\
%                 & Text Data Extraction         & N/A                   & 2                 &               &    \begin{tabular}[c]{@{}c@{}}c: aeroBERT \cite{astroBERT},  \\ SafeAeroBERT \cite{SafeAeroBERT} \end{tabular}                                                           \\
\hline
\multirow{2}{5em}{Coding}            
                & Code Generation        & 3                  & 3                  &    3            &   Codex                                             \\
                 & Debugging     & 3                    &     3               &                &     Codex                                                       \\
\hline
%\begin{tabular}[c]{@{}l@{}}Data\\ Analysis\end{tabular}            & Sentiment Analysis                    & N/A                    & 3                  & N/A              &   b: FinBERT \cite{araci2019finbert}                      \\
%                 & Exploratory Analysis & 1                    &                    &                &         a: ProtGPT2 \cite{ProtGPT2}                                                   \\
%\hline
\multirow{2}{5em}{Writing}          
                 & Writing \& Editing        & 3                    & 3                  & 3              & General LLMs  \\
                 & Outreach \& Education     & 3                    & 3                  & 3              &  General LLMs                                                              \\
%\hline
%\begin{tabular}[c]{@{}l@{}}Decision\\Making\end{tabular}            & --                    &                     &                   &               &                         \\
\hline\hline
\end{tabular}
    \begin{tablenotes}
      \small
      \item Following the rating system by \cite{korinek2023}: 1 = experimental; results are inconsistent and require significant human oversight; 2 = useful; requires oversight but will likely improve workflow; 3 = highly useful; incorporating \acp{LLM} will improve research workflow. These are subjective ratings of \ac{LLM} capabilities provided by authors from their respective scientific fields. In the last column, we give examples of general and domain-specific models that can be used to tackle each tasks. 
    \end{tablenotes}
\end{threeparttable}
} % end of \scalebox
\end{table}
